Probabilistic Search for Structured Data via Probabilistic Programming and Nonparametric Bayes

Databases are widespread, yet extracting relevant data can be difficult. Without substantial domain knowledge, multivariate search queries often return sparse or uninformative results. This paper introduces an approach for searching structured data based on probabilistic programming and nonparametric Bayes. Users specify queries in a probabilistic language that combines standard SQL database search operators with an information theoretic ranking function called predictive relevance. Predictive relevance can be calculated by a fast sparse matrix algorithm based on posterior samples from CrossCat, a nonparametric Bayesian model for high-dimensional, heterogeneously-typed data tables. The result is a flexible search technique that applies to a broad class of information retrieval problems, which we integrate into BayesDB, a probabilistic programming platform for probabilistic data analysis. This paper demonstrates applications to databases of US colleges, global macroeconomic indicators of public health, and classic cars. We found that human evaluators often prefer the results from probabilistic search to results from a standard baseline.

==> figures/ivies.tex <==
%!TEX root = ../main.tex

\begin{figure*}[ht]
\tt\footnotesize
\renewcommand{\ttdefault}{cmtt}
\lstset{
  basicstyle=\ttfamily\footnotesize,
  columns=fullflexible,
  keepspaces=true,
  upquote=true,
  % Define . and % as letters to include them in keywords.
  alsoletter={\.,\%},
  % First type of keywords.
  % Use \bfseries\textcolor{OliveGreen} to get bolded text.
  morekeywords=[1]{SELECT, FROM, ORDER, BY, RELEVANCE, PROBABILITY,
  EXISTING, ROWS, IN, THE, CONTEXT, OF, TO, AS, WHERE, IS, NOT, DESC, LIMIT,
  SELECT, AND, HYPOTHETICAL, ROW},
  keywordstyle=[1]\textcolor{DarkGreen},
  % Add strings
  showstringspaces=False,
  stringstyle=\ttfamily\color{Sepia},
  morestring=[b]",
}

\begin{subfigure}[t]{.325\linewidth}
% Use mdframed to align codebox and table.
\begin{lstlisting}
%bql SELECT
...   "institute",
...   "median_sat_math",
...   "expenditure_on_students",
...   "tuition_fee",
...   "median_student_debt",
...   "admit_rate",
... FROM college_scorecard
... WHERE
...   "admit_rate" > 0.20
... ORDER BY
...   RELEVANCE PROBABILITY
...   TO EXISTING ROWS IN (
...    'Harvard University',
...    'Princeton University',
...    'Yale University',
...    'Duke University',
...   )
...  IN THE CONTEXT OF
...   "expenditure_on_students"
... LIMIT 10
\end{lstlisting}
\end{subfigure}%
\begin{subtable}[t]{.675\linewidth}
\subcaption{Top-ranking universities which are most relevant to Ivy League
schools in the context of ``expenditure on students'', but with significantly
less competitive admissions.}
\label{subtable:college-bql}
\begin{tabular}{lrrrrr}
\toprule
    institute            & sat & expenditure & tuition & debt & admit \\
\midrule
    Carnegie Mellon      & 750      & 31,807   & 49,022  & 25,250 & 24\% \\
    Emory University     & 700      & 40,450   & 45,008  & 19,000 & 26\% \\
    Colgate University   & 700      & 22,975   & 48,175  & 16,115 & 26\% \\
    Univ of Notre Dame   & 725      & 26,632   & 46,237  & 21,250 & 21\% \\
    Boston College       & 690      & 20,571   & 47,436  & 19,000 & 33\% \\
    Santa Clara          & 665      & 12,668   & 43,812  & 20,500 & 49\% \\
    Babson College       & 660      & 14,110   & 45,120  & 27,000 & 26\% \\
    Case Western         & 710      & 30,078   & 43,158  & 24,250 & 38\% \\
    George Washington    & 655      & 20,938   & 48,760  & 25,350 & 43\% \\
    New York Univ.       & 685      & 30,237   & 46,170  & 23,300 & 35\% \\
\bottomrule
\end{tabular}
\includegraphics[width=\linewidth]{assets/scorecard_boxes.pdf}
\end{subtable}
\caption{%
Using relevance probability in BQL to search for universities in the US College
Scorecard dataset
\citep[available at \url{collegescorecard.ed.gov/data}]{council2015}.
%
We are interested in the median math SAT score, yearly tuition, and median
graduating debt at universities which are predictively relevant to Ivy League
schools in the context of ``expenditure on students'', but have an
admission rate of at least 20\%.
%
These metrics for universities shown in \subref{subtable:college-bql} are all
significantly better than national averages, but are still less than Ivy League
schools.}
\label{fig:college}
\end{figure*}


==> figures/satellites.tex <==
%!TEX root = ../main.tex

\begin{figure*}
\section{Application to a dataset of earth satellites from the Union of Concerned Scientists}
\label{appx:satellites}
\tt\footnotesize

\mdfdefinestyle{codeframe}{
  linecolor=white,%
  leftmargin=0,%
  rightmargin=0,%
  innertopmargin=0,%
  innerbottommargin=0,%
  innerleftmargin=0,%
  innerrightmargin=0,%
}

\renewcommand{\ttdefault}{cmtt}
\lstset{
  basicstyle=\ttfamily\footnotesize,
  columns=fullflexible,
  keepspaces=True,
  % Enable single-string ', (requires textcomp package).
  upquote=true,
  % Remove skip above of codebox.
  aboveskip=0pt,
  % Define . and % as letters to include them in keywords.
  alsoletter={\.,\%},
  % First type of keywords.
  % Use \bfseries\textcolor{OliveGreen} to get bolded text.
  morekeywords=[1]{SELECT, FROM, ORDER, BY, RELEVANCE, PROBABILITY,
  EXISTING, ROWS, IN, THE, CONTEXT, OF, TO, AS, WHERE, IS, NOT, DESC, LIMIT,
  SELECT, AND, HYPOTHETICAL, ROW, CREATE, TABLE, POPULATION, FOR, SCHEMA,
  GUESS, STATTYPES, STATISTICAL, TYPES, FOR, METAMODEL, BASELINE,
  ANALYZE, INITIALIZE, MINUTE, MODELS, DEPENDENCE, PROBABILITY, PAIRWISE,
  VARIABLES, LIKE},
  keywordstyle=[1]\textcolor{DarkGreen},
  % Add strings
  showstringspaces=False,
  stringstyle=\ttfamily\color{Sepia},
  morestring=[b]",
}

\begin{subfigure}[t]{.3\linewidth}
\begin{lstlisting}[aboveskip=\medskipamount]
%bql SELECT
...   "name",
...   "country_of_operator",
...   "operator_owner",
...   "purpose"
...  FROM satellites_raw
...  WHERE
...    "purpose"
...     LIKE '%science%'
\end{lstlisting}

\begin{lstlisting}[aboveskip=\medskipamount]
%bql SELECT
...   "name",
...   "country_of_operator",
...   "operator_owner",
...   "purpose",
... FROM satellites
... ORDER BY
...   RELEVANCE PROBABILITY
...   EXISTING ROW ((
...    'Hubble Telescope'
...  ))
...  IN THE CONTEXT OF
...   "country_of_operator"
... LIMIT 10
\end{lstlisting}%
\end{subfigure}
\begin{subtable}[t]{.7\linewidth}
\caption{
Suppose a user is interested in finding the names of the major operators of
satellites whose purpose is scientific research.
%
Then user specifies a search condition
\texttt{"purpose" LIKE '\%science\%'} to filter those satellites which have the
substring ``science'' in their ``purpose'' attribute.
%
Ten records matching this criteria are shown below.
%
A shortcoming of this SQL query is that satellites with science-related purposes
but without the substring ``science'' in their ``purpose'' field do not match
the filter, resulting in many relevant records being omitted from the result
set.}

\label{subfig:satellites-sql}
\begin{tabularx}{\linewidth}{Xrllrrr}
\toprule
make     & price & wheels & doors & engine & horsepower & body \\
\midrule
mercedes & 40,960 & rear   & four  & 308    & 184        & sedan \\
\bottomrule
\end{tabularx}

\bigskip

\subcaption{%
We use
Using the Hubble Telescope result from \subref{subfig:satellites-sql} as a
representative search satellite in a latent concept for ``science'' satellites,
and ranking each existing satellite by its relevance probability to the Hubble.
%
The top matches are all satellites used for scientific research, with
``purpose'' attributes such as ``Scientific Research'', ``Solar Physics'',
``Space Physics'', and ``Meteorology''.
%
These satellites are primarily operated by the European Space Agency, in
collaboration with NASA
Using \texttt{ORDER BY RELEVANCE PROBABILITY} in BQL ranks each car in the table
by its relevance to the user's specifications, which are specified as a
hypothetical row. The top-10 ranked cars by probability of relevance to the
search query, in the context of \texttt{price}, are shown below in the table
below. The user can now inspect further characteristics of this subset of cars,
to find ones that they like best. }
\label{subfig:satellites-bql}
\begin{tabularx}{\linewidth}{Xrllrrr}
\toprule
 make     & price  & wheels & doors & engine & horsepower & body \\
\midrule
 jaguar   & 35,550 & rear   & four  & 258    & 176        & sedan \\
 jaguar   & 32,250 & rear   & four  & 258    & 176        & sedan \\
 mercedes & 40,960 & rear   & four  & 308    & 184        & sedan \\
 mercedes & 45,400 & rear   & two   & 304    & 184        & hardtop \\
 mercedes & 34,184 & rear   & four  & 234    & 155        & sedan \\
 mercedes & 35,056 & rear   & two   & 234    & 155        & convertible \\
 bmw      & 36,880 & rear   & four  & 209    & 182        & sedan \\
 bmw      & 41,315 & rear   & two   & 209    & 182        & sedan \\
 bmw      & 30,760 & rear   & four  & 209    & 182        & sedan \\
 jaguar   & 36,000 & rear   & two   & 326    & 262        & sedan \\
\bottomrule
\end{tabularx}
\end{subtable}

\caption{A session in BayesDB for probabilistic model building and search in the
satellites dataset \citep{union2016}.}
\label{fig:satellites}

\end{figure*}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

